Serdab: An IoT Framework for Partitioning Neural Networks Computation across Multiple Enclaves

Recent advances in Deep Neural Networks (DNN) and Edge Computing have made it possible to automatically analyze streams of videos from home/security cameras over hierarchical clusters that include edge devices, close to the video source, as well as remote cloud compute resources. However, preserving the privacy and confidentiality of users' sensitive data as it passes through different devices remains a concern to most users. Private user data is subject to attacks by malicious attackers or misuse by internal administrators who may use the data in activities that are not explicitly approved by the user. To address this challenge, we present Serdab, a distributed orchestration framework for deploying deep neural network computation across multiple secure enclaves (e.g., Intel SGX). Secure enclaves provide a guarantee on the privacy of the data/code deployed inside it. However, their limited hardware resources make them inefficient when solely running an entire deep neural network. To bridge this gap, Serdab presents a DNN partitioning strategy to distribute the layers of the neural network across multiple enclave devices or across an enclave device and other hardware accelerators. Our partitioning strategy achieves up to 4.7x speedup compared to executing the entire neural network in one enclave.

==> background.tex <==
\section{Background}\label{sec:background}

\subsection{Trusted Execution Environment (TEE)}
Trusted Execution Environment such as Software Guard Extensions (SGX~\cite{}) is available on Intel processors starting with Skylake. TEE provides a secure area in the processor that protects code and data from all other previleged software on the platform. The code in the TEE is executed safely on secret data that nobody outside the TEE can have access to it including the hardware vendor (e.g., Intel). The privacy and integrity of the code/data inside the TEE is enforced by the hardware. TEEs are sometimes called enclaves and we use both terms interchangably in this paper. Intel SGX supports remote attestation of the code and data in the TEE. This enables a remote user to verify the trustworthiness of the hardware and the integrity of the TEE contents (i.e., code and data). 

%make up the initial state of the enclave. This enables a remote
%user to verify that the initial code and data matching a given
%cryptographic hash are loaded into a genuine enclave. Remote attestation is always the first step in bootstrapping a secure channel to an enclave.

\subsection{Neural Networks}
{\bf Neural Network (NN) Architecture}: A neural network consists of a series of connected
layers that can process a high-dimensional input image and
output a simpler representation. Each layer of a convolutional NN corresponds to a step in computation: these layers include convolutional layers (that combine nearby pixels via convolution operators), pooling
layers (that reduce the dimensionality of the subsequent layers), rectified linear unit (ReLU) layers (that perform a non-linear transformation),
fully connected layers (that performs matrix addition, multiplications), and a softmax layer (that outputs the final prediction based on the previous layers. 


%As illustrated below [1], combining multiple such layers in a “deep” architecture and by fitting the appropriate weights of the computation (i.e., the “neurons”) between stages, NNs can learn the structure of common objects and detect their presence
%and absence in a given image. Depending on the task, the best model architecture (e.g., configuration
%of layers) varies, but the overwhelming trend has been to build
%deeper models given more training data.


{\bf NN Training}: Training NNs consists of fitting appropriate weights to a given architecture such that the overall empirical error on a given set of labeled training data is minimized. This process is computationally
expensive, but is now supported by a wide range of software
frameworks such as Google TensorFlow, Torch and Caffe. To train an object detector on video, we would first label a portion of a video (or set of videos) by hand, marking which frames contained cars and which did not. Subsequently, we would feed each frame to a NN training framework. Due to the computational cost of training NNs, companies and researchers have also published hundreds of pre-trained models, each representing thousands of hours of CPU and GPU training time. 


{\bf NN Inference} Applying NNs to video —i.e., inference on video— consists almost exclusively of passing individual video frames to a NN, one frame at a time. That is, to detect objects in video, we evaluate the NN repeatedly, once per frame. In our system, we focus on optimizing the NN inference. For example, we decide on which video frames to feed to a pre-trained object detection/classification model and we decide which part of the NN inference is executed on the private/local compute resources (i.e., edge) and which part is executed in the remote compute resources (i.e., cloud) 



\subsection{Design guidelines}
The above user requirements motivates several key requirements for an IoT platform that allows composition and execution of applications across multiple edge/cloud devices that have secure enclaves. We note that devices that does not have a secure enclave can also be leveraged by the platform and they can process non-privacy-sensitive parts on the application but the requirements of the platform are inspired by the presence of hardware enclaves in a subset of the machines. The following are the key requirements of the platform:

\begin{itemize}
    \item {\bf Dataflow Composition Model}. Data-driven IoT applications are well-suited for a dataflow programming model, where user tasks are vertices in a directed acyclic graphs (DAG) and links represent the dataflow dependency  between the tasks, where a link from task $t_1$ to $t_2$ means that $t_1$ is executed before $t_2$ and the output data of $t_1$ is the input to $t_2$. Many cloud-based data platforms such as Tensorflow, Apache Spark and Apache Storm adopt the dataflow model. Similartly, edge-based data platforms such as Edgent and MiNifi adopt the same concept. Dataflow models simplifies the composition and scheduling of applications because the same task can be used in different applications and compute intensive tasks can be scaled independently to be executed on multiple machines.  
    
      \item {\bf Hardware-agnostic Enclave Application}: Trusted enclaves are manafactured by different hardware vendors such as Intel, ARM and AMD. Their enclave technologies are similar in concept but different in implementation, hardware capabilities, and programming abstractions. Intel's enclave technology is called SGX, and there exist similar technologies such as ARM Trustzone and AMD Secure Encryption Virtualization (SEV). Due to the difference in programming abstractions, enclave application developers have to re-write the application to be compatible with the hardware it runs on. One requirement in IoT platform that supports enclave is to support running a single application on any hardware enclave. This is particularly useful because dataflow tasks in IoT application can be dynamically migrated to different edge devices based on latency and availability requirements. 
      %In order to support hardware-agnostic applications, the platform has to provide a programming abstraction that separate the application logic from the hardware-specific commands that initializes the enclave and sends data to it so that the user (App developer) can focus on writing the task logic (e.g., object detection) and the platform's runtime handles the deployment on different enclave technologies.
      
      \item {\bf Service-oriented Enclave Application}: IoT applications deal with continous streams of data coming from devices such as cameras or sensors. Hence, the tasks that run inside the enclave are not expected to be a monolithic tasks that runs once from start to end but instead the task has to be a service that runs in the background and continously recieves requests that contain encrypted data and responds with an encrypted output after processing. 
      %Ideally, the platform should support different service implementations such as synchrnous services in which the client blocks waiting for the server to responds, or asynchronous services in which the client sends the data to the server through a message queue (e.g., RabbitMQ, Redis) and the server dispatches data from the queue and processes them before writing them back in another queue where the client can recieve the results.
      
      \item {\bf Dataflow between Trusted and Untrusted devices}:
      IoT compute resources are distributed. The resources maybe colocated in the same local area network or spanning multiple geographical locations (e.g., some resources in user location, and some resources in edge/cloud datacenters) so the network connectivity is crucial. In addition, some devices might have hardware enclaves and others does not. Hence, the platform has to manage multiple geo-distributed devices where the data flows from the TEE to the untrusted hardware in the same device and then it travels over a wide area network to another device with trusted hardware. The platform has to ensure end-to-end confidentiality and privacy of the data as it passes from one tusted hardware to another. Additionally, the user needs be able to perform remote attestation on all the trusted hardwares that touches the application in order to ensure code integrity. 
      
       \item {\bf Support for Selective-Trust}: As described in the user requirements, the users need to specify which tasks gets executed in the TEE and which tasks can be executed in the regular CPU. This could be due to the fact that the task is not privacy task or the hardware it runs on is under the user's premises. Hence, the platform needs to provide an abstraction in which the user can manually specify which compute resource in which the tasks is executed on in addition to whether it should be placed in a trusted hardware or not. 
       
       %The platform takes this specifications and handles the deployment of the tasks in the requested hardware and manages the data transfer between tasks.  
       
       
       \item {\bf Privacy-Aware Placement}: The Selective Trust has an assumption that the users can manually specify which tasks should run in the trusted hardware. This approach is feasible for high-level tasks like detecting instrusion in home cameras, however, considering that these tasks are typically implemented as one or a sequence of complex deep learning models where each model has multiple layers, it becomes hard for the user to specify which layers of the deep learning model has to be placed in the trusted hardware. On the other hand, the performance and memory limitations of trsuted hardware (e.g., 128 MB in SGX), makes the trusted hardware in-adequate to efficiently support running an entire deep and complex neural network within an enclave. Hence, a balance has to be taken between running some layers in the enclave until the raw data is concealed and running the rest of the computation on a faster processor or another enclave. This requires the platform to reason about the tradeoff between privacy and latency and to automatically control the placement of neural network layers to maximize both properties. 
     
    
\end{itemize}


